Software Portability for Computer Algebra

We have been involved in the creation of multiple software systems for computer algebra, including Reduce, Maple, Axiom and Aldor as well as a number of smaller specialised programs. We relate observations on how the meaning of software portability has changed over time and how it continues to evolve. We describe how the systems with which we have first-hand experience have achieved portability, how the central issues have changed over time and the challenges that remain.

==> IfExistsUseBBL.tex <==
% If this file exists, then the .bbl file is used instead of calling bibtex.
% It cannot be empty.   To force bibtex to run, rename this file to something else.
